Point3D: tracking actions as moving points with 3D CNNs

Spatio-temporal action recognition has been a challenging task that involves detecting where and when actions occur. Current state-of-the-art action detectors are mostly anchor-based, requiring sensitive anchor designs and huge computations due to calculating large numbers of anchor boxes. Motivated by nascent anchor-free approaches, we propose Point3D, a flexible and computationally efficient network with high precision for spatio-temporal action recognition. Our Point3D consists of a Point Head for action localization and a 3D Head for action classification. Firstly, Point Head is used to track center points and knot key points of humans to localize the bounding box of an action. These location features are then piped into a time-wise attention to learn long-range dependencies across frames. The 3D Head is later deployed for the final action classification. Our Point3D achieves state-of-the-art performance on the JHMDB, UCF101-24, and AVA benchmarks in terms of frame-mAP and video-mAP. Comprehensive ablation studies also demonstrate the effectiveness of each module proposed in our Point3D.

==> SECTIONS/40_Experiments/ab_3D.tex <==
In this ablation study, we explore the design of 3D Head backbone, as shown in Table \ref{tab: ab_3Dbackbone}. Specifically, we employ the 3D backbone with 3D-ResNet with different depths \cite{targ2016resnet} and with other popular 3D-CNN architectures such as MobileNets \cite{howard2017mobilenets, sandler2018mobilenetv2} and ShuffleNet \cite{zhang2018shufflenet, ma2018shufflenet}. We can observe that the stronger 3D Head backbone we use, better the achieved results. This further demonstrates the importance of the proposed 3D Head in our Point3D. 
Moreover, applying the light-weight backbone in our 3D Head achieves the competitive performance compared to the MOC~\cite{li2020actions}. 

\begin{table}[h]
	%\normalem
	\caption{Exploration study on the design of 3D Head backbone.}
	\label{tab: ab_3Dbackbone}
	\renewcommand\tabcolsep{4.0pt}
	\centering
	\scalebox{0.55}{
		\begin{tabular}{c|c|c|c|c|c|c}
			\hline
			\multicolumn{1}{c|}{\multirow{2}{*}{3D backbone}} &
			\multicolumn{1}{c|}{\multirow{2}{*}{FPS}} &\multicolumn{1}{c|}{Frame-mAP(\%)} & \multicolumn{4}{c}{Video-mAP(\%)}                     \\ \cline{4-7} 
\multicolumn{1}{c|}{}   & \multicolumn{1}{c|}{}                    & \multicolumn{1}{c|}{0.5}                                & 0.2  & 0.5  & 0.75 & \multicolumn{1}{c}{0.5:0.95} \\ \hline\hline
            MobileNetV1 2.0x  & \textbf{31}& 67.5 & 72.6 & 71.8 & 64.9 & 53.8 \\
			MobileNetV2 2.0x & \textbf{31}& 69.1 & 75.5 & 73.6 & 66.8 & 55.6 \\
			ShuffleNetV1 2.0x &30 &70.2 & 77.6 & 75.8 & 67.5 & 56.4 \\
			ShuffleNetV2 2.0x &30& 70.8 & 78.9 & 77.5 & 68.1 & 57.6 \\\hline
			ResNet-18 & 27 & 72.6 & 80.4 & 78.5 & 68.4 & 58.3 \\
			ResNet-50 & 25 & 74.5 & 82.5 & 80.3 & 68.7 & 58.8 \\
			ResNet-101 & 20 & 77.4 & 86.5 & 84.2 & 69.4 & 59.8 \\
			ResNeXt-101 & 23 & \textbf{79.2} & \textbf{89.1} & \textbf{86.1} & \textbf{71.5} & \textbf{60.9} \\
			\hline
			\end{tabular}}
\end{table}




==> SECTIONS/40_Experiments/ab_input3D.tex <==
Furthermore, we explore three types of 3D Head input, including the raw clip, frame heatmaps and the output from Point Head, as shown in Table \ref{tab: ab_input3D}. Output from the Point Head achieves better performance against the raw clip and the heatmap alone, which shows the advantage of the Point Head. Combining two of three input types can improve the performance further. Especially, using the raw clip and the output from Point Head achieves the best performance among all input combinations in terms of four video-mAP metrics. Feeding all three types of input into the 3D Head achieves the best frame-mAP, which further demonstrate the flexibility of the proposed Point3D architecture. 


\begin{table}[h]
	%\normalem
	\caption{Exploration study on the type of 3D head input.}
	\label{tab: ab_input3D}
	\renewcommand\tabcolsep{2.0pt}
	\centering
	\scalebox{0.8}{
		\begin{tabular}{c|c|c|c|c|c|c|c}
			\hline
			\multicolumn{1}{c|}{{Raw}} &  \multicolumn{1}{c|}{\multirow{2}{*}{Heatmap}}&
			\multicolumn{1}{c|}{{Point Head}}&
			\multicolumn{1}{c|}{Frame-mAP(\%)} & \multicolumn{4}{c}{Video-mAP(\%)}                     \\ \cline{5-8} 
\multicolumn{1}{c|}{clip}  & & \multicolumn{1}{c|}{output}                        & \multicolumn{1}{c|}{0.5}                                & 0.2  & 0.5  & 0.75 & \multicolumn{1}{c}{0.5:0.95} \\ \hline\hline
			\checkmark & &  & 76.1 & 87.4 & 84.5 & 69.6 & 58.7 \\

			& \checkmark & & 77.9 & 87.9 & 84.8 & 69.9 & 59.1 \\
			&   & \checkmark& 79.2 & 89.1 & 86.1 & 71.5 & 60.9 \\

			\checkmark & \checkmark & & 78.1 & 89.0   & 85.2 & 70.3 & 59.4 \\

			  & \checkmark & \checkmark &  79.4 & 89.3 & 86.2 & 71.7 & 61.1 \\
			 \checkmark&  & \checkmark & 79.5 & \textbf{89.4} & \textbf{86.5} & \textbf{71.8} & \textbf{61.3} \\
			 \checkmark & \checkmark & \checkmark &  \textbf{79.6} & 89.2 & 86.1 & 71.5 & 61.0 \\
			\hline
			\end{tabular}}
\end{table}





==> SECTIONS/40_Experiments/ab_weight.tex <==
In Table \ref{tab: ab_weight}, we ablate $\lambda_1$ and $\lambda_2$, two important parameters in our Point3D to balance the weight of Point Head and 3D Head in the overall loss $L_{overall}$. We see that the performance gap among different settings are small, which further shows the robustness of our Point3D to the weight hyper-parameters. In our case, we set $\lambda_1=10$ and $\lambda_2=1$ to achieve the best performance. 

\begin{table}[h]
	%\normalem
	\caption{Exploration study on $\lambda_1$ and $\lambda_2$.}
	\label{tab: ab_weight}
	\renewcommand\tabcolsep{6.0pt}
	\centering
	\scalebox{0.8}{
		\begin{tabular}{c|c|c|c|c|c|c}
			\hline
			\multicolumn{1}{c|}{\multirow{2}{*}{$\lambda_1$}} & \multirow{2}{*}{$\lambda_2$} & \multicolumn{1}{c|}{Frame-mAP(\%)} & \multicolumn{4}{c}{Video-mAP(\%)}                     \\ \cline{4-7} 
\multicolumn{1}{c|}{}                &       & \multicolumn{1}{c|}{0.5}                                & 0.2  & 0.5  & 0.75 & \multicolumn{1}{c}{0.5:0.95} \\ \hline\hline
            1 & 1  &79.2 & 89.1 & 86.1 & 71.5 & 60.9 \\
            1 & 5  &79.3 & 89.2 & 86.2 & 71.6 & 61.1 \\
            1 & 10 & 79.5 & 89.4 & 86.4 & 71.8 & 61.4 \\
			1 & 15  & 79.1 & 88.9 & 85.9 & 71.3 & 60.8 \\
			5  & 1 & 79.7 & 89.5 & 86.4 & 71.7 & 61.3 \\
			10 & 1 & \textbf{79.9} & \textbf{89.8} & \textbf{86.8} & \textbf{71.9} & \textbf{61.5} \\
			15 & 1 & 79.6 & 89.4 & 86.3 & 71.6 & 61.2 \\
			\hline
			\end{tabular}}
\end{table}



==> SECTIONS/40_Experiments/exp_error.tex <==
In this section, we closely follow \cite{li2020actions,kalogeiton2017action} to conduct an error analysis on the frame mAP in order to better explore our proposed Point3D. Specifically, we investigate five kinds of action detection errors as described in \cite{kalogeiton2017action}, which are localization errors (EL), classification errors (EC), time errors (ET), other errors (EO), and missed detection errors (EM). 
% 1) \textit{classification errors} $E_C$: the detection IoU is greater than 0.5 with the ground-truth box of another action class.
% 2) \textit{localization errors} $E_L$: the detection class is correct in a frame but the bounding box IoU with ground truth is less than 0.5. 
% 3) \textit{time errors} $E_T$: the detection in the untrimmed video covers the frame that doesn't belong to the temporal extent of the current action instance.
% 4) \textit{missed detection errors} $E_M$: cannot detect out a ground truth box. 
% 5) \textit{other errors} $E_O$: the detection appears in a frame without the class and has IoU less than 0.5 with the ground truth bounding box of other classes. 
Among these action detection errors, EL, EC, ET, and EO identify false positive detection and we follow the calculation of frame mAP and measure the area under the curve when plotting the percentage of each category at all recall values.
On the other hand, EM refers to the actions that we fail to detect at all. 
It is computed by measuring the percentage of ground truth boxes for which there are no correct detections.
We report the results for $T=1, 7, 16$ on the JHMDB and UCF$101$-$24$ dataset in Figure~\ref{fig: exp_error}. 

From Figure \ref{fig: exp_error}, we make the following observations: 
\textit{First}, when experimenting with $T=7$ on the JHMDB dataset, we achieve lower EL, EC, EO, and EM than the MOC~\cite{li2020actions} by $0.09\%$, $5.78\%$, $0.07\%$, and $0.20\%$, respectively. Our Point3D outperforms the MOC by $6.14\%$ in terms of frame-mAP. Similar improvements can be seen on the UCF$101$-$24$ dataset. This shows the advantage of our Point3D in spatio-temporal action recognition. 
\textit{Second}, with the increase of $T$, i.e., the length of the input clip, the frame-mAP increases and all the errors except ET decreases. This agrees with the common sense that the length of the input clip is crucial for action recognition. But there is a trade-off between the precision and the speed using different $T$s. We explore this trade-off in Section~\ref{sec: ablation_study}.
\textit{Third}, the increasing gap from $T=1$ to $T=7$ is insignificant compared to the increasing magnitude from $T=1$ and $T=7$. Thus, we set $T=7$ in our case for a better trade-off between the precision and the speed. 

From the error analysis, we can observe that our classification error EC (see the blue bar in Figure~\ref{fig: exp_error}) is still high. 
To explore this error source, we visualize failure cases in the last row in Figure~\ref{fig: exp_visualization}. 
Our Point3D sometimes makes some false positive classifications at initial frames since it is hard to recognize the action before it happens.
% due to the lack of temporal contexts. 
% This is because it is hard to recognize the action before it happens. 

%\red{failure case analysis}

%\red{TO add a bar chart to show error analysis, following Action as moving points.} 

\begin{figure}[!htb]
\setlength{\abovecaptionskip}{-1.5em}
\setlength{\belowcaptionskip}{-1em}
		%\fbox{\rule{0pt}{2in} \rule{0.8\linewidth}{0pt}}
		\centerline{\includegraphics[width=0.7\linewidth]{figs/exp_error.pdf}}
    	\caption{ Error analysis of our Point3D for $T = 1,7,16$
on the JHMDB and UCF101-24  dataset. We show frame-mAP  and different sources of error.}
\vspace{-0.5em}
	\label{fig: exp_error}
\end{figure}




==> SECTIONS/40_Experiments/exp_jhmdb.tex <==
\noindent{\textbf{JHMDB.}} We compare our method to the current state-of-the-art methods, including $2$D backbone methods (Yang \cite{yang2019step}, Song\cite{song2019tacnet}, Zhao \cite{zhao2019dance}, MOC \cite{li2020actions}) and 3D backbone methods (C3D \cite{hou2017tube}, I3D \cite{gu2018ava}, S3D-G \cite{sun2018actor}) with ImageNet \cite{imagenet_cvpr09} pretrain and COCO \cite{lin2014coco} pretrain. Table \ref{tab: sota_jhmdb} shows the results on the JHMDB benchmark. Our method outperforms the state-of-the-art methods by a large margin in terms of both frame-mAP and three video-mAP metrics. Except for video-mAP with a threshold of 0.75 where we achieve a comparable result as the MOC \cite{li2020actions} detector, our Point3D outperforms all other methods present. 





\begin{table}[h]
%\normalem
	\caption{Comparison with the state-of-the-arts on the JHMDB benchmark. ``IN" and ``CC'" indicate models are pre-trained on ImageNet and COCO, respectively. Numbers in bold denote the first place in terms of performance, and underlined numbers denote the second place.}
	\label{tab: sota_jhmdb}
	\renewcommand\tabcolsep{6.0pt}
	\centering
	\scalebox{0.8}{
\begin{tabular}{l|c|cccc}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multicolumn{1}{c|}{Frame-mAP} & \multicolumn{4}{c}{Video-mAP(\%)}                     \\ \cline{3-6} 
\multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.5(\%)}                                & 0.2  & 0.5  & 0.75 & \multicolumn{1}{c}{0.5:0.95} \\ \hline\hline
\multicolumn{2}{l}{2D detector}                                \\ \hline
%Saha                                          & -                                                   & 72.6 & 71.5 & 43.3 & 40.0                          \\ 
Peng \cite{peng2016multi}                                          & 58.5                                                 & 74.3 & 73.1 &  -   &  -       \\  
Singh \cite{singh2017online}                                         & -                                                    & 73.8 & 72   & 44.5 & 41.6                          \\ 
Kalegeiton \cite{kalogeiton2017action}                                    & 65.7                                                 & 74.2 & 73.7 & 52.1 & 44.8                          \\ 
%Yang                                          & -                                                   &  -   &  -   & -    & -                            \\ 
Song \cite{song2019tacnet}                                          & 65.5                                                 & 74.1 & 73.4 & 52.5 & 44.8                          \\ 
Zhao \cite{zhao2019dance}                                          & -                                                   &  -   & 74.7 & 53.3 & 45.0                          \\ 
MOC \cite{li2020actions} (IN)                                           & 68.0                                                 & 76.2 & 75.4 & 68.5 & 54.0                          \\ 
MOC \cite{li2020actions} (CC)                                           & 70.8                                                 & 77.3 & 77.2 & \textbf{71.7} & 59.1                          \\ \hline\hline
\multicolumn{2}{l}{3D detector}                             \\ \hline
C3D \cite{hou2017tube}                                           & 61.3                                                 & 78.4 & 76.9 &  -   &  -                           \\ 
I3D \cite{gu2018ava}                                           & 73.3                                                 &  -   & 78.6 &  -   &  -                           \\ 
S3D-G \cite{sun2018actor}                                         & \underline{77.9}                                                 &  -   & 80.1 &  -   &  -                            \\ \hline\hline
\multicolumn{2}{l}{2D+3D detector}                                                               &      &      &      &                               \\ \hline
YOWO \cite{kopuklu2019yowo}                                          & 74.4                                                 & \underline{87.8} & \underline{85.7} & 58.1 &  -                            \\ 
Point3D (IN)                                &                                           76.4 & 86.8 & 84.1 & 69.8 & \underline{59.3} \\
Point3D (CC)                                &                 \textbf{78.1} & \textbf{88.2} & \textbf{85.6} & \underline{70.8} & \textbf{60.4}      \\ \hline
\end{tabular}}
\end{table}

==> SECTIONS/40_Experiments/exp_runtime.tex <==
Following previous work~\cite{li2020actions} closely, we evaluate the two-stream offline speed of our Point3D's  on a single Tesla V100 GPU. Point3D reaches a competitive speed of 20 fps compared with existing 2D detectors. In Figure~\ref{fig: exp_runtime}, we compare our Point3D with some current state-of-the-art methods which have reported their speed in the original paper~\cite{li2020actions, kopuklu2019yowo, zhao2019dance, yang2019step, kalogeiton2017action, singh2017online, saha2017amtnet}. Point3D achieves the best performance against the existing methods in terms of video mAP within reasonable runtime. This further confirms the advantages of our Point3D in tracking action as moving points with 3D-CNNs. 

\begin{figure}[!htb]
\setlength{\abovecaptionskip}{-1.5em}
\setlength{\belowcaptionskip}{-1em}
		%\fbox{\rule{0pt}{2in} \rule{0.8\linewidth}{0pt}}
		\centering
		\includegraphics[width=0.5\linewidth]{figs/exp_run_time.pdf}
    	\caption{Runtime comparison with the state-of-the-art methods using video mAP with a threshold of 0.2 and FPS of frame per second. A high video mAP (in red) and a small FPS (in blue) indicates a better performance. Results of \cite{saha2017amtnet} are omitted as their video mAP is much lower compared to other methods. }
    	%\blue{[update axis map to mAP, remove Saha results]}
    	\vspace{-1em}
	\label{fig: exp_runtime}
\end{figure}

==> SECTIONS/40_Experiments/exp_ucf101.tex <==
\noindent{\textbf{UCF101-24.}} We compare our method with the state-of-the-art methods in Table \ref{tab: sota_ucf}. Our Point3D outperforms the current state-of-the-art methods by a significant margin over all metrics. This direct comparisons demonstrate the improvement using Point3D. Introducing the 3D Head in Point3D helps to outperform the 2D detectors \cite{peng2016multi, singh2017online, kalogeiton2017action, song2019tacnet, zhao2019dance, li2020actions} by a large margin. We also achieve a better performance than YOWO \cite{kopuklu2019yowo} with the 3D detector with the help of our Point Head that tracks actions as moving points. 



\begin{table}[h]
%\normalem
	\caption{Comparison with the state-of-the-art approaches on the UCF101-24 benchmark. ``IN" and ``CC" indicate models are pre-trained on ImageNet and COCO respectively. Numbers in bold denote the first place in terms of performance, and underlined numbers denote the second place.}
	\label{tab: sota_ucf}
	\renewcommand\tabcolsep{4.0pt}
	\centering
	\scalebox{0.8}{
\begin{tabular}{l|c|ccccc}
\hline
\multirow{2}{*}{Method} & {Frame-mAP} & \multicolumn{5}{c}{Video-mAP(\%)}          \\ \cline{3-7} 
\multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.5(\%)}  & 0.1    & 0.2   & 0.5   & 0.75  & 0.5:0.95 \\ \hline\hline
\multicolumn{2}{l}{2D detector}                   \\ \hline
Saha \cite{saha2017amtnet}                    & -                                &   -     & 66.7  & 35.9  & 7.9   & 14.4     \\ 
Peng \cite{peng2016multi}                    & 39.9                            & 50.4   & 42.3  &  -   &  -   &  -     \\ 
Singh \cite{singh2017online}                   & -                                &  -      & 73.5  & 46.3  & 15.0  & 20.4     \\ 
Kalegeiton \cite{kalogeiton2017action}              & 69.5                            &   -     & 76.5  & 49.2  & 19.7  & 23.4     \\ 
Yang \cite{yang2019step}                    & 75.0                            &    -    & 76.6  &  -  &   - &   -     \\
Song \cite{song2019tacnet}                    & 72.1                            &   -     & 77.5  & 52.9  & 21.8  & 24.1     \\ 
Zhao \cite{zhao2019dance}                    & -                                &   -     & 78.5  & 50.3  & 22.2  & 24.5     \\ 
MOC \cite{li2020actions} (IN)                     & 76.9                            &   -     & 81.3  & 54.4  & 29.5  & 28.4     \\ 
MOC \cite{li2020actions} (CC)                      & 78.0                            &   -     & \underline{82.8}  & 53.8  & 29.6  & 28.3     \\ \hline\hline
\multicolumn{2}{l}{3D detector}        \\ \hline
C3D \cite{hou2017tube}                     & 41.4                            &   -     & 47.1  &  -  &  -   & -     \\ 
I3D \cite{gu2018ava}                     & 76.3                            &   -     &  -   & 59.9  &  -  & -       \\  \hline\hline
\multicolumn{2}{l}{2D+3D detector}    \\ \hline
YOWO \cite{kopuklu2019yowo}  & 80.4                            & 82.5   & 75.8  & 48.8  &   -   &  -      \\ 
Point3D (IN)          &                  \underline{81.2} & \underline{83.7} & 82.6 & \underline{54.6} & \underline{31.2} & \underline{30.5} \\
Point3D (CC)          &      \textbf{83.5} & \textbf{85.4} & \textbf{84.5} & \textbf{55.1} & \textbf{33.4} & \textbf{31.8} \\\hline
\end{tabular}}
\end{table}

==> SECTIONS/REBUTTAL/R1.tex <==


\noindent{\textbf{R1-Q1.}} 
We have checked each line the manuscript and fixed all typos in the updated version.





==> SECTIONS/REBUTTAL/R2.tex <==

\noindent{\textbf{R2-Q1.}}
For knot-point annotations used at the training, we take the original 2D coordinates annotations of the knot-points from open-source dataset. For datasets without annotations, we implement an open-source tool OpenPose (Cao \textit{et al} TPAMI'2019) to extract the 2d coornidates of knot points as labels.
% \textcolor{red}{From the backbone information we could predict several knot points. Besides predicting the location of knot points, distance between center point and each knot point is also predicted. So with the location and the distance, each knot point can be converted to predicted center point. We use predicted center points to calculate loss.}

\noindent{\textbf{R2-Q2.}}
The heatmap of knot points help localize the 2d coordinates of knot points in each frame. The distance of knot points from the center point along the x and y axes are used to refine the location of the center point and generate a bounding box of the actor at the localization.

\noindent{\textbf{R2-Q3.}}
We also used the knot points at the inference time.
\textcolor{red}{Both center point and knot point are used for localization but with it yields different performance.}
As we reported in Table 3, adding knot points further boosts the performance of bbox detection in terms of frame-mAP \textcolor{red}{which shows the importance of knot points}. 

\noindent{\textbf{R2-Q4.}}
Inspired by CFAM module in YOWO, we calculate the temporal information attention across frames in TWA to capture the long-range dependencies for action classification. TWA is not the main novelty of our Point3D, but can be used to boost the final performance of our Point3D. We have validated the effectiveness of TWA in Table 3, where adding TWA to CP+KP and CP+KP+3D Head further increases the frame-mAP by 2.0\% and 1.1\%.

\noindent{\textbf{R2-Q5.}}
Thanks for your insightful suggestion. We are working on the direction by incorporating the knot-point information into action classification part for the next version of our Point3D.

% \textcolor{red}{\noindent{\textbf{R2-Q6.}}
% Actually we use information from backbone (e.g. hourglass structure) to both generate Knot-Point and perform action classification. Knot-Point and Center-Point are used for localization while features from backbone are used for classification.}

==> SECTIONS/REBUTTAL/R3.tex <==
\noindent{\textbf{R3-Q1.}} 
We conduct extensive ablation studies to explore each part of our Point3D in Table 3. As we can see, adding KP to the only CP detector increases the frame-mAP by 0.4\%, while adding KP to (CP+3D head) further increases the frame-mAP by 1.3\%.
This demonstrates the effectiveness of the KP detector in bbox detection. On the other hand, adding KP to the only CP detector increases the video-mAP of four IoU thresholds (0.2, 0.5, 0.75, 0.5:0.95) by 1.3\%, 1.1\%, 0.8\%, and 0.2\%, while adding KP to (CP+3D Head) further increases the video-mAP by 2.6\%, 2.9\%, 0.1\%, and 0.6\%.
This shows the advantage of the KP detector on temporal localization. 					

\noindent{\textbf{R3-Q2.}}
Sorry for causing the confusion. For the UCF dataset without the ground-truth knot points, we implement an open-source tool OpenPose (Cao \textit{et al} TPAMI'2019) to extract the 2d coornidates of knot points as labels. We added the description to the revised version.



==> SECTIONS/REBUTTAL/manuscript.tex <==
We thank reviewers for their insightful and positive feedback.
We are encouraged that they found our idea to be reasonable (\textbf{R1}, \textbf{R2}, \textbf{R3}), our experiments to be thorough and extensive (\textbf{R1}, \textbf{R2}, \textbf{R3}), and our results to be strong (\textbf{R1}, \textbf{R2}, \textbf{R3}).
We address all reviewers’ concerns below and will incorporate all feedback.

\input{SECTIONS/REBUTTAL/R1}


\input{SECTIONS/REBUTTAL/R2}


\input{SECTIONS/REBUTTAL/R3}



